Steering LLMs toward Korean Local Speech: Iterative Refinement Framework for Faithful Dialect Translation

Standard-to-dialect machine translation remains challenging due to a persistent dialect gap in large language models and evaluation distortions inherent in n-gram metrics, which favor source copying over authentic dialect translation. In this paper, we propose the dialect refinement (DIA-REFINE) framework, which guides LLMs toward faithful target dialect outputs through an iterative loop of translation, verification, and feedback using external dialect classifiers. To address the limitations of n-gram-based metrics, we introduce the dialect fidelity score (DFS) to quantify linguistic shift and the target dialect ratio (TDR) to measure the success of dialect translation. Experiments on Korean dialects across zero-shot and in-context learning baselines demonstrate that DIA-REFINE consistently enhances dialect fidelity. The proposed metrics distinguish between False Success cases, where high n-gram scores obscure failures in dialectal translation, and True Attempt cases, where genuine attempts at dialectal translation yield low n-gram scores. We also observed that models exhibit varying degrees of responsiveness to the framework, and that integrating in-context examples further improves the translation of dialectal expressions. Our work establishes a robust framework for goal-directed, inclusive dialect translation, providing both rigorous evaluation and critical insights into model performance.

==> table/table1_ver2.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabularx}{0.95\textwidth}{@{}p{2.8cm} YY c c c@{}}
\hline
Variants & Forms & Analysis / Key Features & BLEU & chrF++ & \textbf{DFS} \\
\hline

\makecell[tl]{\textbf{Source}\\(Standard)} &
제주도는 특별한 약초들이 많이 없으니까 그냥 그냥 넘긴 거 같아 &
Standard grammar and vocabulary. & -- & -- & -- \\

\makecell[tl]{\textbf{Reference}\\(\textit{Jeju} Dialect)} &
제주도는 특별한 약초들이 많이 \underline{엇이난} 그냥 그냥 넘긴 거 \underline{닮아} &
Contains target dialectal features.(\underline{-엇이난} (-eo-si-nan), \underline{-닮아} (-dal-ma)) & -- & -- & -- \\ \hline

\textbf{Hypothesis 1} &
제주도는 특별한 약초들이 많이 없으니깐 그냥 그냥 넘긴 거 같아 &
\textbf{False Success}: Output mirrors the standard source rather than the intended dialect. &
\textbf{52.54} & \textbf{67.82} & -0.672 \\

\textbf{Hypothesis 2} &
제주도\underline{엔} 특별한 약초\underline{덜}이 많이 \underline{읎응께} 그냥 그냥 넘긴 거 같아 &
\textbf{True Attempt}: Generates multiple dialectal features (\underline{-엔} (-en), \underline{-덜} (-deol), \underline{-읎응께} (-eup-eung-kke)) &
27.78 & 36.80 & \textbf{0.672} \\


\hline
\end{tabularx}

%\smallskip
%\raggedright\textit{(*shared meaning: They probably just passed on Jeju island because there aren't many special medicinal herbs.)}

\small \caption{Evaluation distortions in dialect translation: while n-gram metrics favor surface overlap (\textbf{False Success}), the proposed DFS metric accurately captures the shift toward the dialectal output (\textbf{True Attempt}). Underlined morphemes denote dialectal expressions in the reference and hypothesis. The shared meaning is `\textit{I think they just passed on Jeju Island since it doesn't have a lot of special medicinal herbs there.}'}
\label{tab:false_success_analysis}
\end{table*}

==> table/table4_backup.tex <==
% \usepackage{booktabs}  % preamble
\begin{table*}[t]
\renewcommand{\arraystretch}{1.25}
\centering
\caption{Data size 300 — avg\_dlr\_trained vs avg\_dlr\_vanilla (rows = models, columns = methods)}
\label{tab:dlr_trained_vanilla_300}
\small
\begin{tabular}{@{}l *{12}{r}@{}}
\toprule
\multirow{2}{*}{\textbf{Model}}
& \multicolumn{2}{c}{\textbf{ICL}}
& \multicolumn{2}{c}{\textbf{ICL\_CIL\_S}}
& \multicolumn{2}{c}{\textbf{ICL\_CLS\_M}}
& \multicolumn{2}{c}{\textbf{ZS}}
& \multicolumn{2}{c}{\textbf{ZS\_CIL\_S}}
& \multicolumn{2}{c}{\textbf{ZS\_CLS\_M}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}
& \textit{trained} & \textit{vanilla}
& \textit{trained} & \textit{vanilla}
& \textit{trained} & \textit{vanilla}
& \textit{trained} & \textit{vanilla}
& \textit{trained} & \textit{vanilla}
& \textit{trained} & \textit{vanilla} \\
\midrule
HyperCLOVAX & -0.30 & -0.01 & -0.24 & -0.01 & -0.06 &  0.00 & -0.37 & -0.01 & -0.37 & -0.01 & -0.32 & -0.01 \\
Llama-3.1   & -0.26 & -0.01 & -0.24 & -0.01 & -0.10 &  0.00 & -0.37 & -0.01 & -0.37 & -0.01 & -0.32 & -0.01 \\
EEVE        & -0.26 & -0.01 & -0.23 & -0.01 & -0.05 &  0.00 & -0.38 & -0.01 & -0.37 & -0.01 & -0.28 & -0.01 \\
EXAONE-3.5  & -0.04 &  0.00 &  0.07 &  0.00 &  0.27 &  0.00 & -0.39 & -0.01 & -0.32 & -0.01 & -0.08 & -0.01 \\
Gemini-1.5  &  0.31 &  0.00 &  0.36 &  0.00 &  0.39 &  0.00 &  0.36 &  0.00 &  0.38 &  0.00 &  0.40 &  0.00 \\
\bottomrule
\end{tabular}
\end{table*}


==> table/table5_backup.tex <==
\begin{table*}[t!]
\centering
\small
% \setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}llcccccc@{}}
\toprule
\textbf{Metric} & \textbf{Method} & \textbf{HyperCLOVAX} & \textbf{Llama-3.1} & \textbf{EEVE} & \textbf{EXAONE-3.5} & \textbf{Gemini-1.5} & \textbf{Model Avg} \\
\midrule
\multirow{6}{*}{\textbf{chrF++}} 
 & ZS         & 60.33 & 68.97 & 54.03 & 29.05 & 39.50 & 50.38 \\
 & ZS\_CIL\_S & 60.76 & 62.52 & 52.41 & 29.94 & 38.03 & 48.73 \\
 & ZS\_CIL\_M & 52.52 & 44.29 & 39.82 & 25.20 & 38.55 & 40.08 \\
 & ICL        & 59.17 & 71.31 & 70.99 & 65.41 & 63.08 & 65.99 \\
 & ICL\_CIL\_S& 55.35 & 70.42 & 70.48 & 60.19 & 62.13 & 63.72 \\
 & ICL\_CIL\_M& 46.00 & 66.15 & 65.67 & 54.95 & 61.68 & 58.89 \\
\midrule
\multirow{6}{*}{\textbf{BLEU}} 
 & ZS         & 47.64 & 58.53 & 41.71 & 11.44 & 23.06 & 36.48 \\
 & ZS\_CIL\_S & 47.94 & 49.82 & 39.49 & 11.97 & 21.92 & 34.23 \\
 & ZS\_CIL\_M & 38.82 & 28.98 & 25.24 &  8.13 & 22.13 & 24.66 \\
 & ICL        & 46.21 & 61.75 & 61.34 & 52.88 & 49.10 & 54.25 \\
 & ICL\_CIL\_S& 41.44 & 60.57 & 60.68 & 45.75 & 47.73 & 51.23 \\
 & ICL\_CIL\_M& 31.70 & 54.67 & 54.30 & 39.14 & 47.22 & 45.41 \\
\midrule
\multirow{6}{*}{\textbf{DFS}} 
 & ZS         & -0.37 & -0.37 & -0.38 & -0.39 &  0.36 & -0.23 \\
 & ZS\_CIL\_S & -0.37 & -0.37 & -0.37 & -0.32 &  0.38 & -0.21 \\
 & ZS\_CIL\_M & -0.32 & -0.32 & -0.28 & -0.08 &  0.40 & -0.12 \\
 & ICL        & -0.30 & -0.26 & -0.26 & -0.04 &  0.31 & -0.11 \\
 & ICL\_CIL\_S& -0.24 & -0.24 & -0.23 &  0.07 &  0.36 & -0.06 \\
 & ICL\_CIL\_M& -0.06 & -0.10 & -0.05 &  0.27 &  0.39 &  0.09 \\
\midrule
\multirow{6}{*}{\textbf{TDR}} 
 & ZS         & 0.031 & 0.029 & 0.017 & 0.009 & 0.932 & 0.204 \\
 & ZS\_CIL\_S & 0.036 & 0.031 & 0.027 & 0.083 & 0.982 & 0.232 \\
 & ZS\_CIL\_M & 0.076 & 0.084 & 0.131 & 0.424 & 0.994 & 0.342 \\
 & ICL        & 0.093 & 0.152 & 0.156 & 0.414 & 0.852 & 0.334 \\
 & ICL\_CIL\_S& 0.149 & 0.178 & 0.194 & 0.600 & 0.972 & 0.419 \\
 & ICL\_CIL\_M& 0.411 & 0.360 & 0.420 & 0.937 & 0.990 & 0.624 \\
\midrule
\multirow{6}{*}{\textbf{Attempt}} 
 & ZS         & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 & ZS\_CIL\_S & 2.93 & 2.94 & 2.96 & 2.92 & 1.09 & 2.57 \\
 & ZS\_CIL\_M & 2.90 & 2.90 & 2.88 & 2.70 & 1.03 & 2.48 \\
 & ICL        & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
 & ICL\_CIL\_S& 2.76 & 2.67 & 2.66 & 2.01 & 1.19 & 2.26 \\
 & ICL\_CIL\_M & 2.50 & 2.42 & 2.38 & 1.45 & 1.10 & 1.97 \\
\bottomrule
\end{tabular}
\caption{Performance comparison of five language models across six methodologies, evaluated with five key metrics. All scores are averaged over three target dialects (Gyeongsang, Jeolla, and Jeju). The `Model Avg' column on the far right presents the average performance across all models for each method.}
\label{tab:full_results}
\end{table*}

